On Efficient Algorithms For Partial Quantifier Elimination

Earlier, we introduced Partial Quantifier Elimination (PQE). It is a $\mathit{generalization}$ of regular quantifier elimination where one can take a $\mathit{part}$ of the formula out of the scope of quantifiers. We apply PQE to CNF formulas of propositional logic with existential quantifiers. The appeal of PQE is that many problems like equivalence checking and model checking can be solved in terms of PQE and the latter can be very efficient. The main flaw of current PQE solvers is that they do not $\mathit{reuse}$ learned information. The problem here is that these PQE solvers are based on the notion of clause redundancy and the latter is a $\mathit{structural}$ rather than $\mathit{semantic}$ property. In this paper, we provide two important theoretical results that enable reusing the information learned by a PQE solver. Such reusing can dramatically boost the efficiency of PQE like conflict clause learning boosts SAT solving.

==> f3ootnote.tex <==
In our previous papers on PQE solving we just mentioned the
restriction on the order in which assignments are made. However, we
did not describe any implementation problems.


==> junk.tex <==

\vspace{20pt}

%just something to fill out the page
\clearpage
just something to fill out the page
\clearpage


==> s1torage.tex <==
 Since
$D_1$ is the only active D-sequent so far, every clause of $U_1$ is
either present in the formula or is satisfied by \pent{q}{^*}. Then,
from Lemma~\ref{lem:reuse}, it follows that $D_1$ holds in subspace
\pent{q}{^*}.
-------
As mentioned above, for the sake of clarity, we assume that D-sequents
are generated by \Dpqe.
-------
The lemma below is employed in the proof of
Proposition~\ref{prop:main_mult}.
%
% Lemma
%
\begin{lemma}
\label{lem:reuse}
Let $C$ be a clause of \prob{X}{F}. Let $D$ denote an extended
D-sequent \Oods{q}{U}{C} such that no clause of $U$ is satisfied by
\pnt{q}. Let \pent{q}{'} be an assignment such that $\pent{q}{'}
\supset \pnt{q}$. Then $D$ can be safely used in subspace \pent{q}{'}
even if some clauses of $U$ are satisfied by \pent{q}{'}.
\end{lemma}
\begin{proof}
As we showed in~\cite{qe_learn}, $D$ holds in subspace \pnt{q} if all
clauses of $U$ are still present in \prob{X}{F}. Since the extended
D-sequents are constructive, from Proposition~\ref{prop:main_sngl} it
follows that $D$ holds in subspace \pent{q}{'} as well.
\end{proof}
-----------
This makes the
redundancy of $C$ in formula \prob{X}{F \wedge K} in subspace \pnt{q}
obvious.
--------
$\pent{q}{'} \supseteq
\pnt{q}$ $\blacksquare$
----------
\subsection{Some background}
Information on QE in propositional logic can be found
in~\cite{blocking_clause,cav09,cav11,cmu,nik2,cadet_qe}.  QE by
redundancy based reasoning is presented in~\cite{fmcad12,fmcad13}.
One of the merits of such reasoning is that it allows to introduce
\ti{partial} QE.  A description of PQE algorithms and their sources
can be found in~\cite{hvc-14,cav23,cert_tech_rep,ds_pqe,eg_pqe_plus}.
--------------
Given a \ti{decision} PQE
problem, a PQE solver \ti{also} tries to prove a subset of clauses $G$
redundant in a formula \prob{X}{F(X,Y)}, but the goal here is to solve
the problem rather than optimize the formula \prob{X}{F}.
---------
%
% the decision version of PQE
%
\begin{definition}
\label{def:dec_vers} Given a formula \prob{X}{F(X,Y))} and $G$ where
$G \subseteq F$, the \tb{decision version of PQE} is to check if $G$
is redundant in \prob{X}{F} \ie if $\prob{X}{F}\equiv \prob{X}{F
  \setminus G}$.
\end{definition}
-------
One can single
out two kinds of atomic D-sequents for a clause $C$: conflict and
non-conflict ones.  A conflict D-sequent is derived if a conflict
occurs in subspace \pnt{q} and a conflict clause falsified by \pnt{q}
is added to \prob{X}{F}. (This \ti{makes} $C$ redundant in \prob{X}{F}
subspace \pnt{q}.)  A non-conflict D-sequent is derived if $C$ is
\ti{proved} redundant in subspace \pnt{q} without adding a conflict
clause. 
---------
First, many old problems
like equivalence checking, model checking, and SAT and new problems
like property generation can be solved in terms of PQE.
--------
From now on, we will talk about D-sequent reusing without employing a
qualifier (``conflict'' or ``non-conflict'').
-
(So, $K$ indeed implies $C$ in subspace \pnt{q}).
------------
Given a formula \prob{X}{F}, assume a PQE solver derives only extended
D-sequents. Then any derived D-sequent \Oods{q}{U}{C} can be safely
reused in subspace $\pent{q}{^*} \supseteq \pnt{q}$ unless a D-sequent
\oDs{\pent{q}{'}}{U'}{C'} was applied earlier where $C' \in U$ and $C
\in U'$ (and $\pent{q}{^*} \supseteq \pent{q}{'}$).
-
Unfortunately, to avoid circular reasoning, \cite{qe_learn} imposed
severe limitations on reusing multiple D-sequents. In this section, we
\ti{lift those limitations}. Arguably, this will make reusing extended
D-sequents dramatically more effective.
------------------
\begin{proposition}
  \label{prop:main_sngl}
Let \Oods{q}{U}{C} be a constructive D-sequent stating the redundancy
of a clause $C$ in \prob{X}{F} in subspace \pnt{q}. Assume that its
derivation may involve D-sequents stating redundancy of clauses other
than $C$. Then this D-sequent still can be safely reused even if it
does not have.
\end{proposition}
---------
(Note that two D-sequents $D_i$
and $D_j$ with different order numbers may assert redundancy of the
same clause of $F$ but in different subspaces.)
---
Let $C$ be a clause of a formula $F$.  Let \oods{r}{C} and \oods{s}{C}
be D-sequents that hold for \prob{X}{F} and that can be resolved on a
variable $v$.  Let these D-sequents have the scale-down property. Then
the D-sequent \oods{q}{C} obtained by resolving these D-sequents on
$v$ has the scale-down property too.
-----
The constructive D-sequents have the scale-down property.
----------------
Let \Oods{q}{U}{C} be a D-sequent stating the redundancy of a clause
$C$ in \prob{X}{F} in subspace \pnt{q}.Assume that every clause of
the construction set $U$ is either present in \prob{X}{F} in subspace
\pnt{q} or is satisfied by \pnt{q}.  Then \Oods{q}{U}{C} has the
scale-down property.
----------------
\begin{lemma}
\label{lem:align}
Let \oods{q}{C} be a D-sequent that holds for a formula
\prob{X}{F(X,Y)} where $C$ is a quantified clause of $F$. Then this
D-sequent also holds for any formula \prob{X}{F'} obtained from
\prob{X}{F} by adding clauses implied by $F$.
\end{lemma}
\begin{proof}
The fact that \oods{q}{C} holds means that \cof{C}{q} is redundant in
\prob{X}{\cof{F}{q}}. Denote \cof{C}{q} as $C^*$ and \cof{F}{q} as
$F^*$. Redundancy of $C^*$ in \prob{X}{F^*} means that there is no
full assignment \pnt{y} to $Y$ such that \cof{F^*}{y} is unsatisfiable
and \cof{(F^* \setminus \s{C^*})}{y} is satisfiable. In other words,
the fact that \cof{F^*}{y} is unsatisfiable implies that \cof{(F^*
  \setminus \s{C^*})}{y} is unsatisfiable too. The same is true if
$F^*$ is replaced with \cof{F'}{q} .
\end{proof}
---------
The D-sequent \ods{\emptyset}{C_0} of Example~\ref{exmp:scale_down}
does not scale down since it is \ti{not} constructive.
----------
\begin{proposition}
  \label{prop:main_sngl}
Assume a PQE solver derives only constructive D-sequents.  Then every
D-sequent produced by this solver \ti{has the scale-down property}.
\end{proposition}
-------------
Hence, the D-sequent
\ods{\pent{q}{'}}{C_0} does \ti{not} hold for \prob{X}{F} even though
$\pent{q}{'} \supseteq \pnt{q}$ $\blacksquare$
--------
So, the D-sequent \oods{q}{C_0}
holds for \prob{X}{F} where $\pnt{q}=\emptyset$.
------
Before defining constructive D-sequents, we provide definitions for
atomic D-sequents and the operation of resolution of D-sequents.  Some
examples of atomic D-sequents and resolving D-sequents were given in
Subsection~\ref{ssec:pqe_exmp}.
-----------
\subsection{Conflict and non-conflict D-sequents}
Consider the PQE problem of taking a set of clauses $G$ out of
\prob{X}{F(X,Y)}.  Let $C$ be a clause of $G$ whose redundancy is not
proved yet in the current branch of \Dpqe. Suppose that a conflict
occurs in subspace \pnt{q} and $K$ is the conflict clause added to
\prob{X}{F}.  Then \Dpqe derives a \tb{``conflict''} D-sequent stating
the redundancy of $C$ in \prob{X}{F} in any subspace where $K$ is
falsified. If the redundancy of $C$ is proved without encountering a
conflict (\eg $C$ is blocked in subspace \pnt{q}), a \tb{non-conflict}
D-sequent is derived stating the redundancy of $C$ in subspace
\pnt{q}.

One can relate conflict D-sequents with local \ti{inconsistency} and
non-conflict D-sequents with local \ti{unobservability}.  We mean that
if a clause is redundant in \prob{X}{F} in subspace \pnt{q} without
adding new clauses, it does not affect the result of solving the PQE
problem at hand in subspace \pnt{q}. So, $C$ is ``unobservable''
there. Appendix~\ref{app:unobs} shows how non-conflict D-sequents can
express the unobservability of a subcircuit in a subspace. Conflict
D-sequents can be easily reused because inconsistency is a
\ti{semantic} property. (If a formula $R$ is unsatisfiable and $R'
\equiv R$, then formula $R'$ is unsatisfiable too.) Reusing
non-conflict D-sequents is not trivial, because redundancy and hence
unobservability is a \ti{structural} rather than semantic
property. (The fact that a clause $C$ is redundant in formula $R$ and
$R' \equiv R$ \ti{does not} imply that $C$ is redundant in $R'$ too.)
--------
The current PQE algorithms implement redundancy based reasoning via
the machinery of D-sequents~\cite{fmcad12,fmcad13}. A D-sequent is a
record \olds{X}{F}{q}{C} stating the redundancy of a clause $C$ in the
current formula \prob{X}{F} in subspace \pnt{q}. Here \pnt{q} is an
assignment to variables of $F$ and 'D' stands for 'Dependency'.  The
redundancy of $C$ above also holds in any formula \prob{X}{F^*} where
$F^*$ is obtained from $F$ by adding clauses implied by $F$.  For the
sake of simplicity, we will represent a D-sequent as \oods{q}{C}
assuming that the missing parameter \prob{X}{F} is the \ti{current}
formula or some formula \prob{X}{F^*} above.
---------
A major flaw of current PQE solvers is as follows. As we show in
Section~\ref{sec:reuse_pqe}, one can relate conflict D-sequents with
local \ti{inconcistency} and non-conflict D-sequents with local
\ti{unobservability}.  Conflict D-sequents can be easily reused
because inconsistency is a \ti{semantic} property. On the other hand,
reusing non-conflict D-sequents is not trivial, because
unobservability is a \ti{structural} property. So, the current PQE
solvers \tb{do not reuse} non-conflict D-sequents.  Importantly, the
overwhelming majority of derived D-sequents are usually non-conflict
ones and current PQE algorithms repeatedly derive the same
D-sequents. So, not reusing D-sequents cripples the performance of PQE
solving. The main contribution of this paper is adressing the issue of
D-sequent reusing. Namely, we present important theoretical results
enabling safe reusing of D-sequents. These results are presented for
the notion of an \ti{extended} D-sequent introduced
in~\cite{qe_learn}.
---------
although the contents of
these sections apply to any algorithm based on the machinery of
D-sequents.
---------
Consider the D-sequents \ods{\pent{q}{'}}{C} and \ods{\pent{q}{''}}{C}
where $\pent{q}{'}\!=\!(x_0\!=\!0,x_1\!=\!1,x_2\!=\!1)$ and
$\pent{q}{''}\!=\!(x_0\!=\!0,x_1\!=\!0,x_3\!=\!0)$.  The conditionals
\pent{q}{'} and \pent{q}{''} have exactly one variable that is
assigned differently in them (namely $x_1$). So, these D-sequents can
be resolved on $x_1$. The result of resolution is the D-sequent
\oods{q}{C} where $\pnt{q}\!=\!(x_0\!=\!0,x_2\!=\!1,x_3\!=\!0)$.
-
Finally, we adapt Definition~\ref{def:res_of_dseqs} of \tb{resolution}
to extended D-sequents. Let \oDs{\pent{q}{'}}{U'}{C} and
\oDs{\pent{q}{''}}{U''}{C} be extended D-sequents. As before, we
assume that precisely one variable $v$ of $\V{\pent{q}{'}} \cap
\V{\pent{q}{''}}$ has different values in \pent{q}{'} and
\pent{q}{''}. Let \pnt{q} be equal to
$\pent{q}{'}\!\cup\!\pent{q}{''}$ minus assignments to $v$. Then the
D-sequent \Oods{q}{U}{C} where $U\!=\!U'\!\cup U''$ is said to be
obtained by resolution on $v$.
------
Let \ods{\pent{q}{'}}{C} and \ods{\pent{q}{''}}{C} be two
D-sequents.
---------
First, let us explain how the conditional of an atomic D-sequent is
built.  If a condition of Definition~\ref{def:atomic} is met, \Dpqe
derives a D-sequent \Oods{r}{U}{C} where \pnt{r} is a smallest subset
of \pnt{q} for which this condition still holds.  Assume, for
-------
Here \pnt{r}
is a smallest subset of \pnt{q} still satisfying $C$.
--------
(see Remark~\ref{rem:shorten} of the previous section)
---------
So, in this section, we recall
the relevant definitions of~\cite{qe_learn}.
--
Below, we recall an extended definition of a D-sequent introduced
in~\cite{qe_learn} to avoid circular reasoning.
--------
The main problem of D-sequent reusing is that it may lead to
\ti{circular reasoning}.  To address this problem, the definition of a
D-sequent was \ti{extended} in~\cite{qe_learn}.
-----
*) add a lemma about constructive extended D-sequents
-------
Namely, we show that the
\ti{constructive} D-sequents (produced by the existing algorithms
based on D-sequents) do have the scale-down property.
---------
In section~\ref{sec:reuse_dseqs} we present some experimental
results demostrating that a PQE solver \ti{without} D-sequent reusing
repeatedly derives the same D-sequents.
-----------
(Sections~\ref{sec:reuse_pqe}-\ref{sec:mltpl_dseqs}).
----------
*) write a section on decision making
*) write a section on minimizing the
   set of targets
-----------   
That is if a clause $C$ becomes unit in the current
subspace and the only unassigned variable is
--
performing PQE as one global computation (rather than a collection of
local ones).
---------
In
Appendix~\ref{app:reuse_dseqs} we show that a PQE solver repeatedly
generates the same D-sequents. So D-sequent reusing could dramatically
boost its performance.
--------
\footnote{The fact that a clause $C$ if redundant in a formula
  $R$ and that formula $R'$ is logically equivalent to $R$ does not
  imply that $C$ is redundant in $R'$ as well.}.
  -------
(Sections~\ref{sec:reuse_pqe}-\ref{sec:mltpl_dseqs})

